Distribution Discrepancy and Feature Heterogeneity for Active 3D Object Detection

LiDAR-based 3D object detection is a critical technology for the development of autonomous driving and robotics. However, the high cost of data annotation limits its advancement. We propose a novel and effective active learning (AL) method called Distribution Discrepancy and Feature Heterogeneity (DDFH), which simultaneously considers geometric features and model embeddings, assessing information from both the instance-level and frame-level perspectives. Distribution Discrepancy evaluates the difference and novelty of instances within the unlabeled and labeled distributions, enabling the model to learn efficiently with limited data. Feature Heterogeneity ensures the heterogeneity of intra-frame instance features, maintaining feature diversity while avoiding redundant or similar instances, thus minimizing annotation costs. Finally, multiple indicators are efficiently aggregated using Quantile Transform, providing a unified measure of informativeness. Extensive experiments demonstrate that DDFH outperforms the current state-of-the-art (SOTA) methods on the KITTI and Waymo datasets, effectively reducing the bounding box annotation cost by 56.3% and showing robustness when working with both one-stage and two-stage models.

==> Figure/Figure6.tex <==
\begin{figure}[!h]
  \centering
  \hspace*{\fill}
  \begin{subfigure}{0.31\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figure/PVRCNN-active_round.png}
    \caption{}
    \label{fig:6-a}
  \end{subfigure}\hfill % Add some horizontal space between figures
  \begin{subfigure}{0.31\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figure/DDFHGMM.png}
    \caption{}
    \label{fig:6-b}
  \end{subfigure} % Add some horizontal space between figures
  \begin{subfigure}{0.31\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figure/DDFHKDE.png}
    \caption{}
    \label{fig:6-c}
  \end{subfigure}\hfill % Add some horizontal space between figures
  \hspace*{\fill}
  \vspace{-1mm}
  \caption{(a) report 3D mAP of various AL methods on KITTI in each active round. (b-c) represents the impact of different density estimation methods and varying parameter settings on the performance of DDFH.
  }
  \vspace{-5mm}
  \label{fig:5}
\end{figure}

==> Figure/Figure7.tex <==
\vspace{-4mm}
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{Figure/PVRCNN_CLS.png}
    \caption{3D mAP(\%) of DDFH and the AL Baseline across various categories on the KITTI dataset at the moderate difficulty with PV-RCNN.}
    \label{fig:7}
    \vspace{-4mm}
\end{figure}



==> Figure/Figure8.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{Figure/SECOND_KITTI.png}
    \caption{3D mAP(\%) of DDFH and AL baselines on the KITTI val split with SECOND.}
    \label{fig:8}
    \vspace{-4mm}
\end{figure}



==> Figure/Figure9_rebuttal.tex <==
\begin{figure}[!h]
  \centering
  \hspace*{\fill}
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figure/waymo_level_1_second.png}
    \caption{}
    \label{fig:5-a}
  \end{subfigure}\hfill % Add some horizontal space between figures
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figure/waymo_level_2_second.png}
    \caption{}
    \label{fig:5-b}
  \end{subfigure} % Add some horizontal 
  \hspace*{\fill}
  \caption{3D APH of various AL methods on different difficulties with SECOND model in the Waymo dataset.  }
  \vspace{-2mm}
  \label{fig:9_rebuttal}
\end{figure}

==> Table/table1_rebuttal.tex <==
\begin{table}[!h]
\centering
\caption{Compare 3D mAP(\%) scores for general AL and AL for detection in KITTI Dataset with two-stage 3D detector PV-RCNN when acquiring
approximately 1\% queried bounding boxes. †
indicates the reported performance of the backbone
trained with the 100\% labeled set.}
\vspace{1mm}
\scalebox{0.75}{
%\renewcommand{\arraystretch}{1}
\begin{tabular}{@{}clcccccccccccc@{}}
\toprule
& & \multicolumn{3}{c}{AVERAGE} & \multicolumn{3}{c}{CAR} & \multicolumn{3}{c}{PEDESTRIAN} & \multicolumn{3}{c}{CYCLIST} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
& Method & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard \\ 
\midrule
%& ENTROPY& 75.94 & 62.87 & 57.80 & 91.95 & 80.75 & 75.07 & 57.63 & 49.65 & 44.12 & 78.25 & 58.20 & 54.20 \\
%& BALD          &                74.42 &                    62.07 &                57.20 &            91.99 &                81.14 &            75.88 &                   55.68 &                       46.85 &                   41.62 &                75.58 &                    58.21 &                54.11 \\
\multirow{3}{*}{\rotatebox[origin=c]{90}{Generic}} & CORESET \cite{sener2018active}& 72.26 & 59.81 & 55.59 & 87.77 & 77.73 & 72.95 & 47.27 & 41.97 & 38.19 & 81.73 & 59.72 & 55.64 \\
& BADGE \cite{Ash2020Deep} & 75.34 & 61.44 & 56.55 & 89.96 & 75.78 & 70.54 & 51.94 & 40.98 & 45.97 & 84.11 & 62.29 & 58.12 \\
& LLAL \cite{yoo2019learning} & 73.94 & 62.95 & 58.88 & 89.95 & 78.65 & 75.32 & 46.94 & 45.97 & 45.97 & 75.55 & 60.35 & 55.36 \\

\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{AL Detection}} & LT/c \cite{kao2019localization} & 75.88 & 63.23 & 58.89 & 88.73 & 78.12 & 74.87 & 55.17 & 48.37 & 43.63 & 83.72 & 63.21 & 59.16 \\
& Mc-REG \cite{luo2023exploring} & 66.21 & 54.41 & 51.70 & 88.85 & 76.21 & 73.87 & 35.82 & 31.81 & 29.79 & 73.98 & 55.23 & 51.85 \\
& Mc-MI \cite{feng2019deep} & 71.19 & 57.77 & 53.81 & 86.28 & 75.58 & 71.56 & 41.05 & 37.50 & 33.83 & 86.26 & 60.22 & 56.04 \\
& CONSENSUS \cite{schmidt2020advanced} & 75.01 & 61.09 & 57.60 & 90.14 & 78.01 & 74.28 & 56.43 & 49.50 & 44.80 & 78.46 & 55.77 & 53.73 \\
& CRB \cite{luo2023exploring}      &                79.06 &                    66.49 &                61.76 &            90.81 &                79.06 &            74.73 &                   62.09 &                       54.56 &                   48.89 &                84.28 &                    65.85 &                61.66 \\
& CRB(offi.) & 80.70 & 67.81 & 62.81 & 90.98 & 79.02 & 74.04 & 64.17 & 50.82 & 50.82 & 86.96 & 67.45 & 63.56 \\
& KECOR \cite{luo2023kecor}      &                79.81 &                    67.83 &                62.52 &            91.43 &                79.63 &            74.41 &                   63.49 &                       56.31 &                   50.20 &                84.51 &                    67.54 &                62.96 \\
& KECOR(offi.) & 81.63 & 68.67 & 63.42 & 91.71 & 79.56 & 74.05 & 65.37 & 57.33 & 51.56 & 87.80 & 69.13 & 64.65 \\
\midrule
\midrule
& DDFH(Ours) & \textbf{82.27} & \textbf{69.84} & \textbf{64.76} & \textbf{91.76} & \textbf{80.65} & \textbf{76.46} & \textbf{66.37} & \textbf{59.40} & \textbf{52.97} & \textbf{88.68} & \textbf{69.47} & \textbf{64.85} \\
\midrule
\midrule
& PV-RCNN$^\dagger$ & 81.75 & 70.99 & 67.06 & 92.56 & 84.36 & 82.48 & 64.26 & 56.67 & 51.91 & 88.88 & 71.95 & 66.78 \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\label{tab:1}
\end{table}
\FloatBarrier


==> Table/table2_rebuttal.tex <==
\begin{table}[!h]
\centering
\caption{Compare 3D mAP and BEV scores for general AL and AL for detection in KITTI Dataset with one-stage 3D detector SECOND when acquiring
approximately 1\% queried bounding boxes. †
indicates the reported performance of the backbone
trained with the 100\% labeled set.
}
\vspace{1mm}
\scalebox{0.74}{
\renewcommand{\arraystretch}{1}
\begin{tabular}{llcccccc}
\toprule 
 & &  \multicolumn{3}{c}{3D Detection mAP} & \multicolumn{3}{c}{BEV Detection mAP}   \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
Method & Venue &  EASY &  MOD. &  HARD &  EASY &  MOD. &  HARD \\

\midrule
RAND           &    &                66.67 &                    53.15 &                49.12 &                 72.65 &                     60.94 &                 57.12 \\
ENTROPY \cite{wang2014new}        &   {\ttfamily IJCNN'14  } &                69.29 &                    56.58 &                51.59 &                 74.52 &                     63.38 &                 58.65 \\
BALD \cite{gal2017deep}           &   {\ttfamily ICML'17  } &                68.78 &                    55.49 &                50.30 &                 74.21 &                     62.51 &                 57.70 \\
CORESET \cite{sener2018active}        &   {\ttfamily ICLR'18} &                65.96 &                    51.79 &                47.65 &                 73.85 &                     60.22 &                 56.06 \\
LLAL \cite{yoo2019learning}           &   {\ttfamily CVPR'19} &                68.51 &                    56.05 &                50.97 &                 74.57 &                     63.64 &                 58.92 \\
BADGE \cite{Ash2020Deep}          &   {\ttfamily ICLR'20} &                69.09 &                    55.20 &                50.72 &                 75.12 &                     63.05 &                 58.81 \\
BAIT \cite{ash2021gone}          &   {\ttfamily NeurIPS'21} &                69.45 &                    55.61 &                51.25 &                 76.04 &                     63.49 &                 53.40 \\
CRB \cite{luo2023exploring}            &   {\ttfamily ICLR'23} &                71.69 &                    57.16 &                52.35 &                 78.01 &                     64.71 &                 60.04 \\
KECOR \cite{luo2023kecor}        &   {\ttfamily ICCV'23  } &                71.85 &                    57.75 &                52.56 &                 78.30 &                     65.41 &                 60.15 \\
\midrule
\midrule
DDFH(Ours)     &                       &                \textbf{74.13} &                    \textbf{60.61} &                \textbf{55.48} &                 \textbf{79.65} &                     \textbf{67.95} &                 \textbf{63.10} \\
\midrule
\midrule
SECOND$^\dagger$   &                       &                \textbf{78.85} &                    \textbf{68.66} &                \textbf{65.11} &                 \textbf{81.37} &                     \textbf{73.33} &                 \textbf{70.58} \\

\bottomrule
\end{tabular}
}
\label{tab:2}

\end{table}


==> Table/table3_rebuttal.tex <==
%\begin{wraptable}{r}{0.55\textwidth}
\begin{table}[!h]
\centering
% \vspace{-\intextsep}
\vspace{-4.7mm}
\caption{Compare the impact of each component on 3D mAP scores of KITTI dataset at the moderate difficulty}
\scalebox{0.81}{
\renewcommand{\arraystretch}{1}
\begin{tabular}{ccc|c|cccc}
\toprule
DD & FH & CB & LB & Average & Car & Pedes. & Cyclist \\
\midrule
- & - & - & - & 62.97 & 79.44 & 48.93 & 60.52 \\ % RAND
- & - & - & \checkmark & 66.87 & 78.89 & 56.36 & 65.38 \\
- & - & \checkmark & - & 67.69 & 78.41 & 54.96 & \textbf{69.71} \\ % ddfhwcb
- & \checkmark & \checkmark & - & 64.73 & 80.15 & 51.09 & 62.94 \\ % ddfhwodd
\checkmark & - & \checkmark & - & 68.94 & 79.94 & 58.22 & 68.66 \\ % ddfhwofh
\checkmark & \checkmark & - & \checkmark & 67.04 & \textbf{80.95} & 53.99 & 66.19 \\ % ddfhwofh
%\checkmark & \checkmark & - & \checkmark & 67.04 & \textbf{80.95} & 53.99 & 66.19 \\ % ddfhwlb
\midrule
\checkmark & \checkmark & \checkmark & - & \textbf{69.84} & 80.65 & \textbf{59.40} & 69.47 \\ % DDFH(Ours)
\bottomrule
\end{tabular}
}
\label{tab:3}
\vspace{-1mm}
%\end{wraptable}
\end{table}
% =========== 新增 method name like w/o CB ... ============


==> Table/table4.tex <==
\begin{table}[!ht]
\centering
\caption{Compare 3D mAP(\%) scores for different SOTA apporch in KITTI Dataset when acquiring approximately 1\% queried bounding boxes. $^\dagger$ indicates the reported performance of the backbone trained with the 100\% labeled set.}
\vspace{1mm}
\scalebox{0.77}{
%\renewcommand{\arraystretch}{1}
\begin{tabular}{@{}clcccccccccccc@{}}
\toprule
& & \multicolumn{3}{c}{AVERAGE} & \multicolumn{3}{c}{CAR} & \multicolumn{3}{c}{PEDESTRIAN} & \multicolumn{3}{c}{CYCLIST} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
& Method & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard \\ 
\midrule


& CRB \cite{luo2023exploring}      &                79.06 &                    66.49 &                61.76 &            90.81 &                79.06 &            74.73 &                   62.09 &                       54.56 &                   48.89 &                84.28 &                    65.85 &                61.66 \\
& CRB(offi.) & 80.70 & 67.81 & 62.81 & 90.98 & 79.02 & 74.04 & 64.17 & 50.82 & 50.82 & 86.96 & 67.45 & 63.56 \\
& KECOR \cite{luo2023kecor}      &                79.81 &                    67.83 &                62.52 &            91.43 &                79.63 &            74.41 &                   63.49 &                       56.31 &                   50.20 &                84.51 &                    67.54 &                62.96 \\
& KECOR(offi.) & 81.63 & 68.67 & 63.42 & 91.71 & 79.56 & 74.05 & 65.37 & 57.33 & 51.56 & 87.80 & 69.13 & 64.65 \\
& DDFH(Ours) & \textbf{82.27} & \textbf{69.84} & \textbf{64.76} & \textbf{91.76} & \textbf{80.65} & \textbf{76.46} & \textbf{66.37} & \textbf{59.40} & \textbf{52.97} & \textbf{88.68} & \textbf{69.47} & \textbf{64.85} \\
\midrule
\midrule
& PV-RCNN$^\dagger$ & 81.75 & 70.99 & 67.06 & 92.56 & 84.36 & 82.48 & 64.26 & 56.67 & 51.91 & 88.88 & 71.95 & 66.78 \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\label{tab:4}
\end{table}
\FloatBarrier

